XMM-Newton Reflection Grating Spectrometer

The past two decades have witnessed the rapid growth of our knowledge of the X-ray Universe thanks to flagship X-ray space observatories like XMM-Newton and Chandra. A significant portion of discoveries would have been impossible without the X-ray diffractive grating spectrometers aboard these two space observatories. We briefly overview the physical principles of diffractive grating spectrometers as the background to the beginning of a new era with the next-generation (diffractive and non-diffractive) high-resolution X-ray spectrometers. This chapter focuses on the Reflection Grating Spectrometer aboard XMM-Newton, which provides high-quality high-resolution spectra in the soft X-ray band. Its performance and excellent calibration quality have allowed breakthrough advancements in a wide range of astrophysical topics. For the benefit of new learners, we illustrate how to reduce RGS imaging, timing, and spectral data.

==> pocket.tex <==
\subsection{High Energy Transmission Grating Spectrometer}
\label{sct:chandra_hetgs}
High Energy Transmission Grating Spectrometer (HETGS) consists of High Resolution Mirror Assembly (HRMA), High Energy Transmission Grating (HETG), and a focal plane imaging detector. Although other CCD detectors can be used for particular purposes, HETG is designed for use with ACIS-S. With this configuration, considering an on-axis source, the wavelength range of the first-order spectra is $1.2-15$~\AA\ for HEG and $2.5-31$~\AA\ for MEG. The wavelength resolution $\Delta \lambda$ of HEG and MEG is $0.012$~\AA\ and $0.023$~\AA, respectively. Accordingly, the resolving power $R=\lambda/\Delta \lambda$ of HEG and MEG is $65-1070$ and $80-970$, respectively. These are higher than XMM-Newton RGS in the common wavelength range.

Figure~\ref{fig:plot_aeff_hetgs} shows the effective area of HEG and MEG when used with ACIS-S. Over the mission lifetime, the effective area above $\sim10$~\AA\ (or below $\sim1.2$~keV) of ACIS has declined significantly (lowered by at least a factor of $\sim2-3$). This is due to the accumulating out-gassed material on the cold ACIS optical blocking filters\footnote{HRC does not suffer from this issue because it is operated at a warmer temperature.}. Due to the relatively small effective area and energy range, higher order spectra are used less frequently \citep{Chelouche2005, Miller2016}. 

%These two wavelength ranges cover more diagnostic lines of highly ionized ions than RGS, including (1) Lyman series and He-like triplets of cosmic abundance elements like N, O, Ne, Mg, Si, S, Ar, Ca, Fe, and Ni; (2) L-shell transitions of Fe and Ni. 

%-----------------------------Figure----------------------------
\begin{figure}
\centering
\includegraphics[width=\hsize, trim={0.5cm 0.0cm, 0.5cm 0.0cm}, clip]{plot_aeff_hetgs.pdf}
\caption{Effective area of Chandra HEG (blue) and MEG (purple) when used with ACIS-S. Solid and dashed curves are the effective area in 2000 and 2022, respectively. }
\label{fig:plot_aeff_hetgs}
\end{figure}
%-----------------------------Figure------------------------------

\subsection{Low Energy Transmission Grating Spectrometer}
\label{sct:chandra_letgs}
Low Energy Transmission Grating Spectrometer (LETGS) consists of High Resolution Mirror Assembly (HRMA), Low Energy Transmission Grating (LETG), and a focal plane imaging detector. The primary focal plane imaging detector is HRC-S for LETG. With this configuration, considering an on-axis source, the wavelength range of the first-order spectra is $1.2-175$~\AA. The wavelength resolution $\Delta \lambda$ is 0.05~\AA. Accordingly, the resolving power $R=\lambda/\Delta \lambda$ is $60-3500$. Caution that the intrinsic energy resolution of HRC-S is so poor ($E/\Delta E\sim1$) that it cannot be used to separate overlapping spectral orders. Consequently, higher-order features will also appear in the same spectrum. For instance, an Si {\sc xii} line observed at 44.17~\AA\ (first-order) will be accompanied by a third-order line at 14.72~\AA\ \citep{Brinkman2000}. LETGS can also be used with ACIS-S, which will cover a wavelength range of $1.2-60$~\AA. But this configuration has a lower quantum efficiency. 

Figure~\ref{fig:plot_aeff_letgs} shows the effective area of the 1st to 8th order with the HRC-S + LETGS configuration. While the 1st order dominates the effective area, contributions from higher orders are not negligible. They are recommended to be taken into account in the spectral analysis. 


%-----------------------------Figure----------------------------
\begin{figure}
\centering
\includegraphics[width=\hsize, trim={0.5cm 0.0cm, 0.5cm 0.0cm}, clip]{plot_aeff_letgs.pdf}
\caption{Effective area of Chandra LEG when used with HRC-S. The first three orders are shown as solid, dashed, and dotted blue curves. Higher orders are shown in other colors. }
\label{fig:plot_aeff_letgs}
\end{figure}
%-----------------------------Figure------------------------------


% This wavelength range includes diagnostic lines from moderately ionized ions\citep{Mao2017}, such as Be-like Si {\sc xi} , B-like Ne {\sc v}, C-like S {\sc ix}. 
